A Split-Central-Buffered Load-Balancing Clos-Network Switch with In-Order Forwarding

We propose a configuration scheme for a load-balancing Clos-network packet switch that has split central modules and buffers in between the split modules. Our split-central-buffered Load-Balancing Clos-network (LBC) switch is cell based. The switch has four stages, namely input, central-input, central-output, and output stages. The proposed configuration scheme uses a pre-determined and periodic interconnection pattern in the input and split central modules to load-balance and route traffic. The LBC switch has low configuration complexity. The operation of the switch includes a mechanism applied at input and split-central modules to forward cells in sequence. The switch achieves 100\% throughput under uniform and nonuniform admissible traffic with independent and identical distributions (i.i.d.). These high switching performance and low complexity are achieved while performing in-sequence forwarding and without resorting to memory speedup or central-stage expansion. Our discussion includes throughput analysis, where we describe the operations that the configuration mechanism performs on the traffic traversing the switch, and proof of in-sequence forwarding. A simulation study is presented as a practical demonstration of the switch performance on uniform and nonuniform i.i.d. traffic.

==> Reference.tex <==
@inproceedings{chrysos2006scheduling,
  title={Scheduling in Non-Blocking Buffered Three-Stage Switching Fabrics.},
  author={Chrysos, Nikolaos and Katevenis, Manolis},
  booktitle={INFOCOM},
  volume={6},
  pages={1--13},
  year={2006}
}
@inproceedings{kleban2007modified,
  title={The modified {MSM} {C}los switching fabric with efficient packet dispatching scheme},
  author={Kleban, Janusz and Sobieraj, Maciej and Weclewski, Slawomir},
  booktitle={High Performance Switching and Routing, 2007. HPSR'07. Workshop on},
  pages={1--6},
  year={2007},
  organization={IEEE}
}

@inproceedings{kleban2013static,
  title={Static dispatching with internal backpressure scheme for {SMM} {C}los-network switches},
  author={Kleban, Janusz and Suszynska, Urszula},
  booktitle={Computers and Communications (ISCC), 2013 IEEE Symposium on},
  pages={000654--000658},
  year={2013},
  organization={IEEE}
}

@article{sule2018split,
	title={A Split-Central-Buffered Load-Balancing Clos-Network Switch With In-Order Forwarding},
	author={Sule, Oladele Theophilus and Rojas-Cessa, Roberto and Dong, Ziqian and Lin, Chuan-Bi},
	journal={IEEE/ACM Transactions on Networking},
	year={2018},
	publisher={IEEE}
}

@article{theo2018split,
	title={A Split-Central-Buffered Load-Balancing Clos-Network Switch with In-Order Forwarding},
	author={Sule, Oladele Theophilus and Rojas-Cessa, Roberto and Dong, Ziqian and Lin, Chuan-Bi},
	journal={arXiv preprint arXiv:1812.11650},
	year={2018}
}

@inproceedings{pun2002static,
	title={Static round-robin dispatching schemes for Clos-network switches},
	author={Pun, Konghong and Hamdi, Mounir},
	booktitle={High Performance Switching and Routing, 2002. Merging Optical and IP Technologies. Workshop on},
	pages={329--333},
	year={2002},
	organization={IEEE}
}

@article{li2001enhanced,
	title={Enhanced Birkhoff-von Neumann decomposition algorithm for input queued switches},
	author={Li, J and Ansari, N},
	journal={IEE Proceedings-Communications},
	volume={148},
	number={6},
	pages={339--342},
	year={2001},
	publisher={IET}
}

@inproceedings{dixit2013impact,
  title={On the impact of packet spraying in data center networks},
  author={Dixit, Advait and Prakash, Pawan and Hu, Y Charlie and Kompella, Ramana Rao},
  booktitle={INFOCOM, 2013 Proceedings IEEE},
  pages={2130--2138},
  year={2013},
  organization={IEEE}
}

@INPROCEEDINGS{lb-virtual-topologies, 
author={S. M. Irteza and H. M. Bashir and T. Anwar and I. A. Qazi and F. R. Dogar}, 
booktitle={IEEE INFOCOM 2017 - IEEE Conference on Computer Communications}, 
title={Load balancing over symmetric virtual topologies}, 
year={2017}, 
volume={}, 
number={}, 
pages={1-9}, 
keywords={routing protocols;software defined networking;telecommunication network topology;telecommunication traffic;trees (mathematics);SAPS;SDN-based scheme;Symmetric Adaptive Packet Spraying;asymmetric topologies;bisection bandwidth;load balancing algorithm;multirooted trees;packet spraying;symmetric topologies;symmetric virtual topologies;Bandwidth;Conferences;Load management;Network topology;Spraying;Switches;Topology}, 
doi={10.1109/INFOCOM.2017.8057002}, 
ISSN={}, 
month={May},}

@inproceedings{mhamdi2003cbf,
	title={CBF: A high-performance scheduling algorithm for buffered crossbar switches},
	author={Mhamdi, Lotfi and Hamdi, Mounir},
	booktitle={High Performance Switching and Routing, 2003, HPSR. Workshop on},
	pages={67--72},
	year={2003},
	organization={IEEE}
}

@ARTICLE{multipath-switching-slice12, 
author={L. Shi and B. Liu and C. Sun and Z. Yin and L. N. Bhuyan and H. J. Chao}, 
journal={IEEE Transactions on Computers}, 
title={Load-Balancing Multipath Switching System with Flow Slice}, 
year={2012}, 
volume={61}, 
number={3}, 
pages={350-365}, 
keywords={file organisation;probability;resource allocation;MPS;core routers;flow slice;flow-based hashing algorithms;load-balancing multipath switching system;petabit switching capacity;probability;Complexity theory;Context;Delay;Hardware;Switches;Switching systems;Upper bound;Load balancing;switching theory.;traffic measurement}, 
doi={10.1109/TC.2010.279}, 
ISSN={0018-9340}, 
month={March},}

@article{kermani1979virtual,
  title={Virtual cut-through: A new computer communication switching technique},
  author={Kermani, Parviz and Kleinrock, Leonard},
  journal={Computer Networks (1976)},
  volume={3},
  number={4},
  pages={267--286},
  year={1979},
  publisher={Elsevier}
}

@article{birkhoff1946tres,
  title={Tres observaciones sobre el algebra lineal},
  author={Birkhoff, Garrett},
  journal={Univ. Nac. Tucum{\'a}n Rev. Ser. A},
  volume={5},
  pages={147--151},
  year={1946}
}

@misc{lozowick1994method,
  title={Method and apparatus for cut-through data packet transfer in a bridge device},
  author={Lozowick, Philip P and Ben-Michael, Siman-Tov},
  year={1994},
  month=apr # "~26",
  publisher={Google Patents},
  note={US Patent 5,307,345}
}


@article{crrd,
  author =       {E. Oki and Z. Jing and R. Rojas-Cessa and H.J. Chao},
  title =        {Concurrent round-robin-based dispatching schemes for {C}los-network switches},
  journal =    {IEEE/ACM Trans. on Networking.},
  volume=        {10},
  number=        {6},
  year =         {2002},
  pages=         {830-844}
}


@article{rojas2004ufpim,
  title={Captured-frame eligibility and round-robin matching for input-queued packet switches},
  author={Rojas-Cessa, Roberto and Lin, Chuan-Bi},
  journal={IEEE communications letters},
  volume={8},
  number={9},
  pages={585--587},
  year={2004},
  publisher={IEEE}
}

@article{rojas2007captured,
  title={Captured-frame matching schemes for scalable input-queued packet switches},
  author={Rojas-Cessa, Roberto and Lin, Chuan-Bi},
  journal={Computer Communications},
  volume={30},
  number={10},
  pages={2149--2161},
  year={2007},
  publisher={Elsevier}
}

@INPROCEEDINGS{cixb, 
author={R. Rojas-Cessa and E. Oki and Zhigang Jing and H. J. Chao}, 
booktitle={High Performance Switching and Routing, 2001 IEEE Workshop on}, 
title={{CIXB}-1: combined input-one-cell-crosspoint buffered switch}, 
year={2001}, 
pages={324-329}, 
keywords={buffer storage;computational complexity;delays;packet switching;queueing theory;telecommunication traffic;timing;CIXB-1;buffer size;buffered crossbars;combined input-one-cell-crosspoint buffered switch;delay performance;fixed size packets;memory technology;packet switching;pin count;round-robin arbitration;scalability;simulation;switch architecture;switch module;switching throughput;time complexity;timing relaxation;uniform traffic;virtual output queues;Bandwidth;Buffer storage;Chaos;Delay;Fabrics;Rail to rail outputs;Scalability;Switches;Throughput;Traffic control}, 
doi={10.1109/HPSR.2001.923655}, 
}

@inproceedings{cixob,
  title={{CIXOB}-k: Combined input-crosspoint-output buffered packet switch},
  author={Rojas-Cessa, Roberto and Oki, Eiji and Chao, H Jonathan},
  booktitle={Global Telecommunications Conference, 2001. GLOBECOM'01. IEEE},
  volume={4},
  pages={2654--2660},
  year={2001},
  organization={IEEE}
}

@inproceedings{li2005space,
	title={Space-memory-memory architecture for Clos-network packet switches},
	author={Li, Xin and Zhou, Zhen and Hamdi, Mounir},
	booktitle={Communications, 2005. ICC 2005. 2005 IEEE International Conference on},
	volume={2},
	pages={1031--1035},
	year={2005},
	organization={IEEE}
}
@article{ clos1953study,
  title={A Study of Non-Blocking Switching Networks},
  author={Clos, Charles},
  journal={Bell System Technical Journal},
  volume={32},
  number={2},
  pages={406--424},
  year={1953},
  publisher={Wiley Online Library}
}

@article{chang2002load,
  title={Load balanced {B}irkhoff--von {N}eumann switches, part I: one-stage buffering},
  author={Chang, Cheng-Shang and Lee, Duan-Shin and Jou, Yi-Shean},
  journal={Computer Communications},
  volume={25},
  number={6},
  pages={611--622},
  year={2002},
  publisher={Elsevier}
}

@article{changload,
  title={Load balanced {B}irkhoff-von {N}eumann switches, part II: Multi-stage buffering},
  author={Chang, Cheng-Shang and Lee, Duan-Shin and Lien, Ching-Ming},
  publisher={Elsevier}
}

@incollection{ma2007analysis,
  title={Analysis on memory-space-memory {C}los packet switching network},
  author={Ma, Xiangjie and Hu, Yuxiang and Mao, Junpeng and Lan, Julong and Guan, Lian and Zhang, Baisheng},
  booktitle={Advanced Parallel Processing Technologies},
  pages={209--221},
  year={2007},
  publisher={Springer}
}


@inproceedings{rojas2006scalable,
  title={Scalable two-stage {C}los-network switch and module-first matching},
  author={Rojas-Cessa, Roberto and Lin, Chuan-Bi},
  booktitle={2006 Workshop on High Performance Switching and Routing},
  pages={6--pp},
  year={2006},
  organization={IEEE}
}

@article{oki2002concurrent,
  title={Concurrent round-robin-based dispatching schemes for {C}los-network switches},
  author={Oki, Eiji and Jing, Zhigang and Rojas-Cessa, Roberto and Chao, H Jonathan},
  journal={Networking, IEEE/ACM Transactions on},
  volume={10},
  number={6},
  pages={830--844},
  year={2002},
  publisher={IEEE}
}

@inproceedings{oki2009analysis,
  title={Analysis of space-space-space {C}los-network packet switch},
  author={Oki, Eiji and Kitsuwan, Nattapong and Rojas-Cessa, Roberto},
  booktitle={Computer Communications and Networks, 2009. ICCCN 2009. Proceedings of 18th International Conference on},
  pages={1--6},
  year={2009},
  organization={IEEE}
}

@inproceedings{rojas2004maximum,
  title={Maximum weight matching dispatching scheme in buffered {C}los-network packet switches},
  author={Rojas-Cessa, Roberto and Oki, Eiji and Chao, H Jonathan},
  booktitle={Communications, 2004 IEEE International Conference on},
  volume={2},
  pages={1075--1079},
  year={2004},
  organization={IEEE}
}


@inproceedings{dong2012mcs,
  title={{MCS}: buffered {C}los-network switch with in-sequence packet forwarding},
  author={Dong, Ziqian and Rojas-Cessa, Roberto},
  booktitle={Sarnoff Symposium (SARNOFF), 2012 35th IEEE},
  pages={1--6},
  year={2012},
  organization={IEEE}
}

@inproceedings{lin2013minimizing,
  title={Minimizing scheduling complexity with a {C}los-network space-space-memory ({SSM}) packet switch},
  author={Lin, Chuan-Bi and Rojas-Cessa, Roberto},
  booktitle={High Performance Switching and Routing (HPSR), 2013 IEEE 14th International Conference on},
  pages={15--20},
  year={2013},
  organization={IEEE}
}

@inproceedings{dong2011non,
  title={Non-blocking memory-memory-memory {C}los-network packet switch},
  author={Dong, Ziqian and Rojas-Cessa, Roberto},
  booktitle={34th IEEE Sarnoff Symposium},
  pages={1--5},
  year={2011},
  organization={IEEE}
}


@article{hu2010feedback,
  title={Feedback-based scheduling for load-balanced two-stage switches},
  author={Hu, Bing and Yeung, Kwan L},
  journal={IEEE/ACM Transactions on Networking (TON)},
  volume={18},
  number={4},
  pages={1077--1090},
  year={2010},
  publisher={IEEE Press}
}


@article{zhang2014space,
  title={Space-memory-memory {C}los-network switches with in-sequence service},
  author={Zhang, Maosen and Qiu, Zhiliang and Gao, Ya},
  journal={Communications, IET},
  volume={8},
  number={16},
  pages={2825--2833},
  year={2014},
  publisher={IET}
}

@inproceedings{dong2011memory,
  title={Memory-memory-memory {C}los-network packet switches with in-sequence service},
  author={Dong, Ziqian and Rojas-Cessa, Roberto and Oki, Eiji},
  booktitle={High Performance Switching and Routing (HPSR), 2011 IEEE 12th International Conference on},
  pages={121--125},
  year={2011},
  organization={IEEE}
}

@article{chao2003matching,
  title={Matching algorithms for three-stage bufferless {C}los network switches},
  author={Chao, H Jonathan and Jing, Zhigang and Liew, Soung Y},
  journal={Communications Magazine, IEEE},
  volume={41},
  number={10},
  pages={46--54},
  year={2003},
  publisher={IEEE}
}


@article{xia2016practical,
  title={A practical large-capacity three-stage buffered {C}los-network switch architecture},
  author={Xia, Yu and Hamdi, Mounir and Chao, H Jonathan},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={27},
  number={2},
  pages={317--328},
  year={2016},
  publisher={IEEE}
}

@inproceedings{hassen2017high,
  title={High-Capacity {C}los-Network Switch for Data Center Networks},
  author={Hassen, Fadoua and Mhamdi, Lotfi},
  booktitle={IEEE International Conference on Communications 2017},
  year={2017},
  organization={IEEE}
}

@article{lee1997path,
  title={Path switching-a quasi-static routing scheme for large-scale {ATM} packet switches},
  author={Lee, Tony T. and Lam, Cheuk H.},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={15},
  number={5},
  pages={914--924},
  year={1997},
  publisher={IEEE}
}
@inproceedings{chao2005trueway,
  title={Trueway: a highly scalable multi-plane multi-stage buffered packet switch},
  author={Chao, H Jonathan and Park, Jinsoo and Artan, Sertac and Jiang, Shi and Zhang, Guansong},
  booktitle={High Performance Switching and Routing, 2005. HPSR. 2005 Workshop on},
  pages={246--253},
  year={2005},
  organization={IEEE}
}

@article{atlanta,
  title={Low-cost scalable switching solutions for broadband networking: the {ATLANTA} architecture and chipset},
  author={Chiussi, Fabio M and Kneuer, Joseph G and Kumar, Vijay P},
  journal={IEEE Communications Magazine},
  volume={35},
  number={12},
  pages={44--53},
  year={1997},
  publisher={IEEE}
}

@inproceedings{keslassy2002maintaining,
  title={Maintaining packet order in two-stage switches},
  author={Keslassy, Isaac and McKeown, Nick},
  booktitle={INFOCOM 2002. Twenty-First Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
  volume={2},
  pages={1032--1041},
  year={2002},
  organization={IEEE}
}

@book{rojas2016interconnections,
  title={Interconnections for Computer Communications and Packet Networks},
  author={Rojas-Cessa, Roberto},
  year={2016},
  publisher={CRC Press}
}

@article{lee1996new,
	title={A new decomposition algorithm for rearrangeable Clos interconnection networks},
	author={Lee, Hyun Yeop and Hwang, Frank K and Carpinelli, John D},
	journal={IEEE Transactions on Communications},
	volume={44},
	number={11},
	pages={1572--1578},
	year={1996},
	publisher={IEEE}
}

@inproceedings{hu2008joint,
	title={On joint sequence design for feedback-based two-stage switch architecture},
	author={Hu, Bing and Yeung, Kwan L},
	booktitle={High Performance Switching and Routing, 2008. HSPR 2008. International Conference on},
	pages={110--115},
	year={2008},
	organization={IEEE}
}

@inproceedings{mekkittikul1998practical,
	title={A practical scheduling algorithm to achieve 100\% throughput in input-queued switches},
	author={Mekkittikul, Adisak and McKeown, Nick},
	booktitle={INFOCOM'98. Seventeenth Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={2},
	pages={792--799},
	year={1998},
	organization={IEEE}
}

@book{bertsekas1992data,
	title={Data networks},
	author={Bertsekas, Dimitri P and Gallager, Robert G and Humblet, Pierre},
	volume={2},
	year={1992},
	publisher={Prentice-Hall International New Jersey}
}

@article{little1961proof,
	title={A proof for the queuing formula: L= $\lambda$ W},
	author={Little, John DC},
	journal={Operations research},
	volume={9},
	number={3},
	pages={383--387},
	year={1961},
	publisher={INFORMS}
}

@article{chan1997pollaczek,
	title={Pollaczek-Khinchin formula for the M/G/1 queue in discrete time with vacations},
	author={Chan, WC and Lu, T-C and Chen, R-J},
	journal={IEE Proceedings-Computers and Digital Techniques},
	volume={144},
	number={4},
	pages={222--226},
	year={1997},
	publisher={IET}
}

@misc{bronshteinhandbook,
	title={Handbook of Mathematics. 2007},
	author={Bronshtein, IN and Semendyayev, KA and Musiol, G and Muehlig, H},
	publisher={Springer, Berlin}
}

@article{anderson1993high,
	title={High-speed switch scheduling for local-area networks},
	author={Anderson, Thomas E and Owicki, Susan S and Saxe, James B and Thacker, Charles P},
	journal={ACM Transactions on Computer Systems (TOCS)},
	volume={11},
	number={4},
	pages={319--352},
	year={1993},
	publisher={ACM}
}

@article{mckeown1993scheduling,
	title={Scheduling cells in an input-queued switch},
	author={McKeown, Nick and Varaiya, Pravin and Walrand, Jean},
	journal={Electronics Letters},
	volume={29},
	number={25},
	pages={2174--2175},
	year={1993},
	publisher={IET}
}

@article{karol1987input,
	title={Input versus output queueing on a space-division packet switch},
	author={Karol, Mark and Hluchyj, Michael and Morgan, Samuel},
	journal={IEEE Transactions on communications},
	volume={35},
	number={12},
	pages={1347--1356},
	year={1987},
	publisher={IEEE}
}

@article{karol1987input,
	title={Input versus output queueing on a space-division packet switch},
	author={Karol, Mark and Hluchyj, Michael and Morgan, Samuel},
	journal={IEEE Transactions on communications},
	volume={35},
	number={12},
	pages={1347--1356},
	year={1987},
	publisher={IEEE}
}

@phdthesis{mckeown1995scheduling,
	title={Scheduling algorithms for input-queued cell switches},
	author={McKeown, Nicholas William},
	year={1995},
	school={University of California, Berkeley}
}

@article{mekkittikul1997scheduling,
	title={Scheduling VOQ switches under non-uniform traffic},
	author={Mekkittikul, Adisak and McKeown, Nick},
	journal={CSL Technical Report, CSL-TR 97-747},
	year={1997},
	publisher={Citeseer}
}

@inproceedings{dai2000throughput,
	title={The throughput of data switches with and without speedup},
	author={Dai, JG and Prabhakar, Balaji},
	booktitle={INFOCOM 2000. Nineteenth Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={2},
	pages={556--564},
	year={2000},
	organization={IEEE}

}

@inproceedings{mekkittikul1996starvation,
	title={A starvation-free algorithm for achieving 100\% throughput in an input-queued switch},
	author={Mekkittikul, Adisak and McKeown, Nick},
	booktitle={Proc. ICCCN},
	volume={96},
	pages={226--231},
	year={1996},
	organization={Citeseer}
}

@article{jenq1983performance,
	title={Performance analysis of a packet switch based on single-buffered banyan network},
	author={Jenq, Yih-Chyun},
	journal={IEEE Journal on Selected Areas in Communications},
	volume={1},
	number={6},
	pages={1014--1021},
	year={1983},
	publisher={IEEE}
}

@article{dong2012throughput,
	title={Throughput analysis of shared-memory crosspoint buffered packet switches},
	author={Dong, Ziqian and Rojas-Cessa, Roberto},
	journal={IET communications},
	volume={6},
	number={9},
	pages={1045--1053},
	year={2012},
	publisher={IET}
}

@inproceedings{rojas2006combined,
	title={Combined Input-Crosspoint Buffered Packet Switch with Flexible Access to Crosspoints Buffers},
	author={Rojas-Cessa, Roberto and Dong, Ziqian},
	booktitle={Devices, Circuits and Systems, Proceedings of the 6th International Caribbean Conference on},
	pages={255--260},
	year={2006},
	organization={IEEE}
}

@inproceedings{shah2002delay,
	title={Delay bounds for approximate maximum weight matching algorithms for input queued switches},
	author={Shah, Devavrat and Kopikare, Milind},
	booktitle={INFOCOM 2002. Twenty-First Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={2},
	pages={1024--1031},
	year={2002},
	organization={IEEE}
}

@article{bastin2007lyapunov,
	title={Lyapunov stability analysis of networks of scalar conservation laws},
	author={Bastin, Georges and Haut, Bertrand and Coron, Jean-Michel and d Andrea-Novel, Brigitte},
	journal={Networks and Heterogeneous media},
	volume={2},
	number={4},
	pages={749},
	year={2007},
	publisher={AMERICAN INSTITUTE OF MATHEMATICAL SCIENCES}
}

@inproceedings{marsan2001packet,
	title={Packet scheduling in input-queued cell-based switches},
	author={Marsan, F Ajmone and Bianco, Andrea and Giaccone, Paolo and Leonardi, Emilio and Neri, E},
	booktitle={INFOCOM 2001. Twentieth Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={2},
	pages={1085--1094},
	year={2001},
	organization={IEEE}
}

@article{dong2011buffered,
	title={Buffered clos-network packet switch with per-output flow queues},
	author={Dong, Ziqian and Rojas-Cessa, Roberto and Oki, Eiji},
	journal={Electronics letters},
	volume={47},
	number={1},
	pages={32--34},
	year={2011},
	publisher={IET}
}

@inproceedings{cai2011avoiding,
	title={Avoiding speedup from bandwidth overhead in a practical output-queued packet switch},
	author={Cai, Lin and Rojas-Cessa, Roberto and Kijkanjanarat, Taweesak},
	booktitle={Communications (ICC), 2011 IEEE International Conference on},
	pages={1--5},
	year={2011},
	organization={IEEE}
}

@article{chuang1999matching,
	title={Matching output queueing with a combined input/output-queued switch},
	author={Chuang, Shang-Tse and Goel, Ashish and McKeown, Nick and Prabhakar, Balaji},
	journal={IEEE Journal on Selected Areas in Communications},
	volume={17},
	number={6},
	pages={1030--1039},
	year={1999},
	publisher={IEEE}
}

@inproceedings{charny1998algorithms,
	title={Algorithms for providing bandwidth and delay guarantees in input-buffered crossbars with speedup},
	author={Charny, Anna and Krishna, P and Patel, Naimish and Simcoe, Robert},
	booktitle={Quality of Service, 1998.(IWQoS 98) 1998 Sixth International Workshop on},
	pages={235--244},
	year={1998},
	organization={IEEE}
}

@article{krishna1999speedup,
	title={On the speedup required for work-conserving crossbar switches},
	author={Krishna, Pattabhiraman and Patel, Naimish S and Charny, Anna and Simcoe, Robert J},
	journal={IEEE Journal on Selected Areas in Communications},
	volume={17},
	number={6},
	pages={1057--1066},
	year={1999},
	publisher={IEEE}
}

@article{prabhakar1999speedup,
	title={On the speedup required for combined input-and output-queued switching},
	author={Prabhakar, Balaji and McKeown, Nick},
	journal={Automatica},
	volume={35},
	number={12},
	pages={1909--1920},
	year={1999},
	publisher={Elsevier}
}

@inproceedings{stephens1998implementing,
	title={Implementing Distributed Packet Fair Queueing in a scalable switch architecture},
	author={Stephens, Donpaul C and Zhang, Hui},
	booktitle={INFOCOM'98. Seventeenth Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={1},
	pages={282--290},
	year={1998},
	organization={IEEE}
}

@article{hluchyj1988queueing,
	title={Queueing in high-performance packet switching},
	author={Hluchyj, Michael G and Karol, Mark J},
	journal={IEEE Journal on selected Areas in Communications},
	volume={6},
	number={9},
	pages={1587--1597},
	year={1988},
	publisher={IEEE}
}

@inproceedings{iliadis1990performance,
	title={Performance of packet switches with input and output queueing},
	author={Iliadis, Ilias and Denzel, WOLFGANG E},
	booktitle={Communications, 1990. ICC'90, Including Supercomm Technical Sessions. SUPERCOMM/ICC'90. Conference Record., IEEE International Conference on},
	pages={747--753},
	year={1990},
	organization={IEEE}
}

@article{pattavina1993analysis,
	title={Analysis of input and output queueing for nonblocking ATM switches},
	author={Pattavina, Achille and Bruzzi, Giacomo},
	journal={IEEE/ACM Transactions on Networking (TON)},
	volume={1},
	number={3},
	pages={314--328},
	year={1993},
	publisher={IEEE Press}
}

@inproceedings{mckeown1997matching,
	title={Matching output queueing with combined input and output queueing},
	author={McKeown, Nick and Prabhakar, Balaji and Zhu, Mingyan},
	booktitle={PROCEEDINGS OF THE ANNUAL ALLERTON CONFERENCE ON COMMUNICATION CONTROL AND COMPUTING},
	volume={35},
	pages={595--603},
	year={1997},
	organization={Citeseer}
}

@article{del1993performance,
	title={Performance evaluation of input and output queueing techniques in ATM switching systems},
	author={Del Re, Enrico and Fantacci, Romano},
	journal={IEEE Transactions on communications},
	volume={41},
	number={10},
	pages={1565--1575},
	year={1993},
	publisher={IEEE}
}

@article{chen1993scoq,
	title={SCOQ: A fast packet switch with shared concentration and output queueing},
	author={Chen, David X and Mark, Jon W},
	journal={IEEE/ACM Transactions on Networking (TON)},
	volume={1},
	number={1},
	pages={142--151},
	year={1993},
	publisher={IEEE Press}
}

@article{rojas2011load,
	title={Load-balanced combined input-crosspoint buffered packet switches},
	author={Rojas-Cessa, Roberto and Dong, Ziqian},
	journal={IEEE Transactions on Communications},
	volume={59},
	number={5},
	pages={1421--1433},
	year={2011},
	publisher={IEEE}
}

@inproceedings{chang1999service,
	title={On service guarantees for input-buffered crossbar switches: a capacity decomposition approach by Birkhoff and von Neumann},
	author={Chang, Cheng-Shang and Chen, Wen-Jyh and Huang, Hsiang-Yi},
	booktitle={Quality of Service, 1999. IWQoS'99. 1999 Seventh International Workshop on},
	pages={79--86},
	year={1999},
	organization={IEEE}
}

@article{von1953certain,
	title={A certain zero-sum two-person game equivalent to the optimal assignment problem},
	author={Von Neumann, John},
	journal={Contributions to the Theory of Games},
	volume={2},
	pages={5--12},
	year={1953}
}

@inproceedings{chang2000birkhoff,
	title={Birkhoff-von Neumann input buffered crossbar switches},
	author={Chang, Cheng-Shang and Chen, Wen-Jyh and Huang, Hsiang-Yi},
	booktitle={IEEE INFOCOM. Nineteenth Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={3},
	pages={1614--1623},
	year={2000},
	organization={IEEE}
}

@inproceedings{anderson1992high,
	title={High speed switch scheduling for local area networks},
	author={Anderson, Thomas E and Owicki, Susan S and Saxe, James B and Thacker, Charles P},
	booktitle={ACM SIGPLAN Notices},
	volume={27},
	number={9},
	pages={98--110},
	year={1992},
	organization={ACM}
}

@article{mckeown1999islip,
	title={The iSLIP scheduling algorithm for input-queued switches},
	author={McKeown, Nick},
	journal={IEEE/ACM transactions on networking},
	volume={7},
	number={2},
	pages={188--201},
	year={1999},
	publisher={IEEE}
}

@inproceedings{kanizo2009crosspoint,
	title={The crosspoint-queued switch},
	author={Kanizo, Yossi and Hay, David and Keslassy, Isaac},
	booktitle={INFOCOM 2009, IEEE},
	pages={729--737},
	year={2009},
	organization={IEEE}
}

@article{lin2005throughput,
	title={The throughput of a buffered crossbar switch},
	author={Lin, Mingjie and McKeown, Nick},
	journal={IEEE communications Letters},
	volume={9},
	number={5},
	pages={465--467},
	year={2005},
	publisher={IEEE}
}

@article{hu2016iterative,
	title={On Iterative Scheduling for Input-Queued Switches With a Speedup of $2-1/N$},
	author={Hu, Bing and Yeung, Kwan L and Zhou, Qian and He, Chunzhi},
	journal={IEEE/ACM Transactions on Networking},
	volume={24},
	number={6},
	pages={3565--3577},
	year={2016},
	publisher={IEEE}
}

@inproceedings{yan2014hybrid,
	title={Hybrid scheduling algorithm for packet switch architecture},
	author={Yan, Fangfang and Lee, Tony T and Ye, Tong and Hu, Weisheng},
	booktitle={Information Science, Electronics and Electrical Engineering (ISEEE), 2014 International Conference on},
	volume={1},
	pages={346--350},
	year={2014},
	organization={IEEE}
}

@article{rojas2006maximum,
	title={On the maximum throughput of a combined input-crosspoint queued packet switch},
	author={Rojas-Cessa, Roberto and Guo, Zhen and Ansari, Nirwan},
	journal={IEICE transactions on communications},
	volume={89},
	number={11},
	pages={3120--3123},
	year={2006},
	publisher={The Institute of Electronics, Information and Communication Engineers}
}

@inproceedings{rojas2005combining,
	title={Combining distributed and centralized arbitration schemes for combined input-crosspoint buffered packet switches},
	author={Rojas-Cessa, R and Guo, Zhen and Ansari, N},
	booktitle={Networks, 2005. Jointly held with the 2005 IEEE 7th Malaysia International Conference on Communication., 2005 13th IEEE International Conference on},
	volume={2},
	pages={776--770},
	year={2005},
	organization={IEEE}
}


@inproceedings{rojas2005matching,
	title={Matching schemes with captured-frame eligibility for input-queued packet switches},
	author={Rojas-Cessa, Roberto and Lin, Chuan-bi},
	booktitle={Communications, 2005. ICC 2005. 2005 IEEE International Conference on},
	volume={2},
	pages={972--976},
	year={2005},
	organization={IEEE}
}

@article{gao2013distributed,
	title={Distributed weight matching dispatching scheme in MSM Clos-network packet switches},
	author={Gao, Ya and Qiu, Zhiliang and Zhang, Maosen and Jiang, Yongbo},
	journal={IEEE Communications Letters},
	volume={17},
	number={3},
	pages={580--583},
	year={2013},
	publisher={IEEE}
}

@inproceedings{tian2012sequence,
	title={An in-sequence guaranteed space-memory-memory Clos-network architecture},
	author={Tian, Yupeng and Zhang, Xiaoping and Li, Menghan and Zhang, Haixiang},
	booktitle={ICT Convergence (ICTC), 2012 International Conference on},
	pages={354--359},
	year={2012},
	organization={IEEE}
}

@inproceedings{xia2013practical,
	title={On practical stable packet scheduling for bufferless three-stage Clos-network switches},
	author={Xia, Yu and Chao, H Jonathan},
	booktitle={High Performance Switching and Routing (HPSR), 2013 IEEE 14th International Conference on},
	pages={7--14},
	year={2013},
	organization={IEEE}
}
@inproceedings{kleban2013static,
	title={Static dispatching with internal backpressure scheme for SMM Clos-network switches},
	author={Kleban, Janusz and Suszynska, Urszula},
	booktitle={Computers and Communications (ISCC), 2013 IEEE Symposium on},
	pages={000654--000658},
	year={2013},
	organization={IEEE}
}

@inproceedings{lin2008module,
	title={Module-First Matching Schemes for Scalable Input-Queued Space-Space-Space Clos-Network Packet Switches},
	author={Lin, C-B and Rojas-Cessa, Roberto},
	booktitle={Communications, 2008. ICC'08. IEEE International Conference on},
	pages={5669--5673},
	year={2008},
	organization={IEEE}
}

@inproceedings{hu2011module,
	title={A Module Matched First Dispatching algorithm for MSM Clos-network switches},
	author={Hu, Yanlang and Li, Minqi and Zhou, Quan and Li, Jun and Zhang, Yi and Li, Jingling},
	booktitle={Electronics, Communications and Control (ICECC), 2011 International Conference on},
	pages={4086--4089},
	year={2011},
	organization={IEEE}
}

@inproceedings{xia2012module,
	title={Module-level matching algorithms for MSM Clos-network switches},
	author={Xia, Yu and Chao, H Jonathan},
	booktitle={High Performance Switching and Routing (HPSR), 2012 IEEE 13th International Conference on},
	pages={36--43},
	year={2012},
	organization={IEEE}
}

@inproceedings{chao2012improved,
	title={Improved Static Desynchronization scheme for Clos-network switches},
	author={Chao, Che-Hsi and Hsu, Yarsun},
	booktitle={Computing Technology and Information Management (ICCM), 2012 8th International Conference on},
	volume={2},
	pages={659--664},
	year={2012},
	organization={IEEE}
}

@inproceedings{kleban2007packet,
	title={Packet dispatching algorithms with the static connection patterns scheme for three-stage buffered clos-network switches},
	author={Kleban, Janusz and Santos, Hugo},
	booktitle={Communications, 2007. ICC'07. IEEE International Conference on},
	pages={6319--6324},
	year={2007},
	organization={IEEE}
}

@misc{rojas2015space,
	title={Space-space-memory (SSM) Clos-network packet switch},
	author={Rojas-Cessa, Roberto and Lin, Chuan-Bi and Dong, Ziqian},
	year={2015},
	month=mar # "~31",
	publisher={Google Patents},
	note={US Patent 8,995,456}
}

@inproceedings{liu2015fault,
	title={Fault-tolerant cell dispatching for onboard space-memory-memory Clos-network packet switches},
	author={Liu, Kai and Yan, Jian and Lu, Jianhua},
	booktitle={High Performance Switching and Routing (HPSR), 2015 IEEE 16th International Conference on},
	pages={1--6},
	year={2015},
	organization={IEEE}
}

@article{yu2011out,
	title={Out-of-sequence prevention for multicast input-queuing space-memory-memory clos-network},
	author={Yu, Hao and Ruepp, Sarah and Berger, Michael S},
	journal={IEEE Communications Letters},
	volume={15},
	number={7},
	pages={761--763},
	year={2011},
	publisher={IEEE}
}

@inproceedings{al2008concatenating,
	title={Concatenating Packets in Variable-Length Input-Queued Packet Switches with Cell-Based and Packet-Based Scheduling},
	author={Al-Saber, Nabeel A and Oberoi, Saurabh and Pedasanaganti, Taraka and Rojas-Cessa, Roberto and Ziavras, Sotirios G},
	booktitle={Sarnoff Symposium, 2008 IEEE},
	pages={1--5},
	year={2008},
	organization={IEEE}
}

@unpublished{trident,
	note = "Technical Report TR-NRL-180401: TRIDENT: A load-balancing Clos-network Packet Switch with Queues between Input and Central Stages and In-Order Forwarding \url{http://web.njit.edu/~rojasces/technical-reports/trident171201.pdf}"
}


@inproceedings{pun2002static,
	title={Static round-robin dispatching schemes for Clos-network switches},
	author={Pun, Konghong and Hamdi, Mounir},
	booktitle={High Performance Switching and Routing, 2002. Merging Optical and IP Technologies. Workshop on},
	pages={329--333},
	year={2002},
	organization={IEEE}
}

@inproceedings{jacobson2009networking,
	title={Networking named content},
	author={Jacobson, Van and Smetters, Diana K and Thornton, James D and Plass, Michael F and Briggs, Nicholas H and Braynard, Rebecca L},
	booktitle={Proceedings of the 5th international conference on Emerging networking experiments and technologies},
	pages={1--12},
	year={2009},
	organization={ACM}
}

@inproceedings{pan2017modeling,
	title={Modeling CCN Packet Forwarding Engine},
	author={Pan, Tian and Huang, Tao and Li, Cong},
	booktitle={GLOBECOM 2017-2017 IEEE Global Communications Conference},
	pages={1--6},
	year={2017},
	organization={IEEE}
}

@inproceedings{virgilio2013pit,
	title={PIT overload analysis in content centric networks},
	author={Virgilio, Matteo and Marchetto, Guido and Sisto, Riccardo},
	booktitle={Proceedings of the 3rd ACM SIGCOMM workshop on Information-centric networking},
	pages={67--72},
	year={2013},
	organization={ACM}
}

@inproceedings{jacobson2009voccn,
	title={VoCCN: voice-over content-centric networks},
	author={Jacobson, Van and Smetters, Diana K and Briggs, Nicholas H and Plass, Michael F and Stewart, Paul and Thornton, James D and Braynard, Rebecca L},
	booktitle={Proceedings of the 2009 workshop on Re-architecting the internet},
	pages={1--6},
	year={2009},
	organization={ACM}
}

@inproceedings{wang2009energy,
	title={Energy efficient collision aware multipath routing for wireless sensor networks},
	author={Wang, Zijian and Bulut, Eyuphan and Szymanski, Boleslaw K},
	booktitle={2009 IEEE International Conference on Communications},
	pages={1--5},
	year={2009},
	organization={IEEE}
}

@article{ploumidis2017flow,
	title={Flow allocation for maximum throughput and bounded delay on multiple disjoint paths for random access wireless multihop networks},
	author={Ploumidis, Manolis and Pappas, Nikolaos and Traganitis, Apostolos},
	journal={IEEE Transactions on Vehicular Technology},
	volume={66},
	number={1},
	pages={720--733},
	year={2017},
	publisher={IEEE}
}

@inproceedings{le2011multipath,
	title={Multipath routing design for wireless mesh networks},
	author={Le, Long},
	booktitle={2011 IEEE Global Telecommunications Conference-GLOBECOM 2011},
	pages={1--6},
	year={2011},
	organization={IEEE}
}
